XAI-based Feature Ensemble for Enhanced Anomaly Detection in Autonomous Driving Systems

The rapid advancement of autonomous vehicle (AV) technology has introduced significant challenges in ensuring transportation security and reliability. Traditional AI models for anomaly detection in AVs are often opaque, posing difficulties in understanding and trusting their decision making processes. This paper proposes a novel feature ensemble framework that integrates multiple Explainable AI (XAI) methods: SHAP, LIME, and DALEX with various AI models to enhance both anomaly detection and interpretability. By fusing top features identified by these XAI methods across six diverse AI models (Decision Trees, Random Forests, Deep Neural Networks, K Nearest Neighbors, Support Vector Machines, and AdaBoost), the framework creates a robust and comprehensive set of features critical for detecting anomalies. These feature sets, produced by our feature ensemble framework, are evaluated using independent classifiers (CatBoost, Logistic Regression, and LightGBM) to ensure unbiased performance. We evaluated our feature ensemble approach on two popular autonomous driving datasets (VeReMi and Sensor) datasets. Our feature ensemble technique demonstrates improved accuracy, robustness, and transparency of AI models, contributing to safer and more trustworthy autonomous driving systems.

==> Related_Work.tex <==
\vspace{-1mm}
\section{Related Work}\label{sec:related_work}

\mustafa{Add related works and why ours is important.}
%\mustafa{We need to add relevant background }


%One example comes from Reference [11], proposed a solution that is based on the adaptive synthetic (ADASYN) oversampling [12] . 

\textbf{Existing Efforts for Leveraging XAI for IDS:} There are several recent works that started exploring leveraging XAI for IDS~\cite{mahbooba2021explainable,patil2022explainable,islam2019domain,roponena2022towards}. % However, the work~\cite{roponena2022towards} proposed an abstract design for Human in-the-Loop approach for intelligent IDS. 
In particular, the work~\cite{mahbooba2021explainable} used only simple decision tree algorithms for extracting decision rules in IDS only on the KDD benchmark dataset, which is not efficient for large-scale datasets. The work~\cite{patil2022explainable} incorporated LIME to only provide local explanations for a single AI model (SVM in that work) for IDS. The work~\cite{islam2019domain} infused the CIA principle for enhancing the explainability of the AI model on the CICIDS-2017 dataset. In particular, all these works did not explore the  
contribution of each feature on the AI's decision, the attack-specific feature importance, combining global and local explanations, and exploring different types of intrusion datasets which we consider here in our current work.

\textbf{Feature Selection for Intrusion Detection:}
%\mustafa{Add works for feature selection} T
There are several works that focused on investigating effective methods for feature selection~\cite{alazab2012using,MEBAWONDU2020e00497,CICIDS,SENSOR}. In particular, most of the methods focused on either using information gain~\cite{alazab2012using,CICIDS,MEBAWONDU2020e00497}, correlation-based methods~\cite{kamalov2020feature}, or K-best method~\cite{SENSOR,li2021lnnls}. However, all of these methods focus on the features of the dataset and do not take the model into consideration while our XAI-based method is based on the effect of these features on the performance of the AI models. 
This helps in better understanding the decision-making of AI models for IDS.

%Limitation of LIME \url{https://arxiv.org/pdf/2012.00093.pdf}
%% Limitations of : ding an optimal solution to segregate the contribution of each participating feature (sample wise) considering interactions (i.e., correlations among features complicate explanations) among features will aid in better explainability of an individual prediction (i.e., per sample). Besides, to ensure trust, estimating the level of uncertainty in the model will be another extension of this work.ensure trust, estimating the level of uncertainty in the model will be another extension 
%% Decision Trees can be easily read and even resemble a human approach to decision-making by splitting the choice into many small subchoices 
% 

%\vspace{-1mm}
